Scotogenic neutrino masses with gauged matter parity and gauge coupling unification

Building up on previous work we propose a Dark Matter (DM) model with gauged matter parity and dynamical gauge coupling unification, driven by the same physics responsible for scotogenic neutrino mass generation. Our construction is based on the extended gauge group \3311, whose spontaneous breaking leaves a residual conserved matter parity, $M_{P}$, stabilizing the DM particle candidates of the model. A key role is played by the Majorana ${\rm SU(3)_{L}}$-octet leptons, in allowing successful gauge coupling unification and one-loop scotogenic neutrino mass generation. Theoretical consistency allows for a \emph{plethora} of new particles at the $\lsim \mathcal{O}$(10) TeV scale, hence accessible to future collider and low-energy experiments.

==> Makefile <==
FILENAME=ScotoOctet_2021_7_28
LATEX = pdflatex
BIBTEX = bibtex
PDFTOPS = pdftops
AR = acroread
GV = gv
RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"

PSFILE = ScotoOctet_2021_7_28.ps 
PDFFILE = ScotoOctet_2021_7_28.pdf

COPY = if test -r ScotoOctet_2021_7_28.toc; then cp ScotoOctet_2021_7_28.toc ScotoOctet_2021_7_28.toc.bak; fi 
RM = /bin/rm -f

CLEAN=rm -f ScotoOctet_2021_7_28.aux ScotoOctet_2021_7_28.log ScotoOctet_2021_7_28.dvi ScotoOctet_2021_7_28.toc ScotoOctet_2021_7_28.out ScotoOctet_2021_7_28.blg ScotoOctet_2021_7_28.mtc ScotoOctet_2021_7_28.mtc1 ScotoOctet_2021_7_28.rel ScotoOctet_2021_7_28.vrb ScotoOctet_2021_7_28.end ScotoOctet_2021_7_28.spl *.aux *~ \#*

WARNING=egrep -i "(Reference|Citation).*undefined" ScotoOctet_2021_7_28.log ; true

HELP=cat /home/jv/bin/help/MakePDFLatexMakefile.help

main:	ScotoOctet_2021_7_28.tex pdf

pdf:	$(PDFFILE)
	$(WARNING)  

all:	$(PDFFILE) $(PSFILE)
	$(WARNING)  

ps:	$(PSFILE) 
	$(WARNING)

gv:	$(PSFILE)
	$(GV) $(PSFILE) &
	$(WARNING)

	$(WARNING)

ar:	$(PDFFILE)
	$(AR) $(PDFFILE) &

%.pdf:	%.tex
	python3.6 /usr/local/bin/PhysBiblio.exe tex bibliography.bib './ScotoOctet_2021_7_28.tex' './Diagrams/ScotoDia.tex' './Diagrams/Gminus2Dia.tex' './Old versions/ScotoOctet_2020_07_08.tex' './Old versions/ScotoOctet_unification.tex' './Old versions/ScotoOctet_2021_4_30.tex' './Old versions/ScotoOctet_2020_11_24-1.tex' './Old versions/ScotoOctet_2020_06_03.tex' './Old versions/ScotoOctet_2020_10_15-1.tex' './Old versions/ScotoOctet_2021_1_28.tex' './Old versions/ScotoOctet_2020_05_28.tex' './Old versions/ScotoOctet_2021_5_13.tex' './Old versions/ScotoOctet_2020_10_15.tex' './Old versions/ScotoOctet_2021_4_12.tex' './Old versions/ScotoOctet_2020_09_08.tex' './tcilatex.tex' 
	$(COPY);$(LATEX) $<
	egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ;true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
	if [  'cmp -s $*.toc $*.toc.bak'  ]; then $(LATEX) $< ; fi
	$(RM) $*.toc.bak

%.ps:	%.pdf
	$(PDFTOPS) $<

clean:	
	$(CLEAN)

realclean: 	
	$(CLEAN)
	$(RM) $(FILENAME).ps $(FILENAME).pdf $(FILENAME).bbl

help:
	$(HELP)

complete: realclean pdf clean


